Self-Supervised Similarity Learning for Digital Pathology

Using features extracted from networks pretrained on ImageNet is a common practice in applications of deep learning for digital pathology. However it presents the downside of missing domain specific image information. In digital pathology, supervised training data is expensive and difficult to collect. We propose a self-supervised method for feature extraction by similarity learning on whole slide images (WSI) that is simple to implement and allows creation of robust and compact image descriptors. We train a siamese network, exploiting image spatial continuity and assuming spatially adjacent tiles in the image are more similar to each other than distant tiles. Our network outputs feature vectors of length 128, which allows dramatically lower memory storage and faster processing than networks pretrained on ImageNet. We apply the method on digital pathology WSIs from the Camelyon16 train set and assess and compare our method by measuring image retrieval of tumor tiles and descriptor pair distance ratio for distant/near tiles in the Camelyon16 test set. We show that our method yields better retrieval task results than existing ImageNet based and generic self-supervised feature extraction methods. To the best of our knowledge, this is also the first published method for self-supervised learning tailored for digital pathology.

==> supp_material.tex <==
% This is samplepaper.tex, a sample chapter demonstrating the
% LLNCS macro package for Springer Computer Science proceedings;
% Version 2.20 of 2017/10/04
% %
% \documentclass[runningheads]{llncs}
% %
% \usepackage{graphicx}
% \usepackage{placeins}
% \usepackage{bbding}
% \usepackage{amsfonts}
% % Used for displaying a sample figure. If possible, figure files should
% % be included in EPS format.
% %
% % If you use the hyperref package, please uncomment the following line
% % to display URLs in blue roman font according to Springer's eBook style:
% % \renewcommand\UrlFont{\color{blue}\rmfamily}
% \graphicspath{{Images/}}
% \begin{document}
% %

% \begin{figure}[t]

%   \centering
%   \centerline{\includegraphics[width=1.0\linewidth]{}}
  
% \caption{...
% }
% \label{peliGAN}
% %
% \end{figure}


% %
% \end{document}



